T-SaS: Toward Shift-aware Dynamic Adaptation for Streaming Data

In many real-world scenarios, distribution shifts exist in the streaming data across time steps. Many complex sequential data can be effectively divided into distinct regimes that exhibit persistent dynamics. Discovering the shifted behaviors and the evolving patterns underlying the streaming data are important to understand the dynamic system. Existing methods typically train one robust model to work for the evolving data of distinct distributions or sequentially adapt the model utilizing explicitly given regime boundaries. However, there are two challenges: (1) shifts in data streams could happen drastically and abruptly without precursors. Boundaries of distribution shifts are usually unavailable, and (2) training a shared model for all domains could fail to capture varying patterns. This paper aims to solve the problem of sequential data modeling in the presence of sudden distribution shifts that occur without any precursors. Specifically, we design a Bayesian framework, dubbed as T-SaS, with a discrete distribution-modeling variable to capture abrupt shifts of data. Then, we design a model that enable adaptation with dynamic network selection conditioned on that discrete variable. The proposed method learns specific model parameters for each distribution by learning which neurons should be activated in the full network. A dynamic masking strategy is adopted here to support inter-distribution transfer through the overlapping of a set of sparse networks. Extensive experiments show that our proposed method is superior in both accurately detecting shift boundaries to get segments of varying distributions and effectively adapting to downstream forecast or classification tasks.

==> Samples/related_works.tex <==
\section{Related Works}
\subsection{Distribution Shift}
Distribution shift \cite{sugiyama2007covariate} is a challenging situation where the joint distribution of inputs and outputs pairs differs between source and target domains. 
Specifically, we talk about covariate shift \cite{sugiyama2007covariate} here, where feature distribution differs while their functional relations are consistent \cite{bickel2009discriminative, sugiyama2007covariate}. 
Transfer learning or domain adaptation is a common way to alleviate distribution shift and attempts to learn an invariant feature embedding that can reduce the gap between source and target domains. 
Various approaches, including metric-based (or non-parametric) \cite{long2017deep}, adversarial-based \cite{tzeng2017adversarial}, reconstruction-based \cite{wang2018deep} and optimization-based \cite{harrison2020continuous} are proposed.  
Previous works mainly consider a static scenario, where only a source domain and target domain are provided \cite{sugiyama2007covariate,tzeng2017adversarial}. 
Recently, few works extend their setting to evolving domain shift or discrete domain shift problems, which is more challenging and more practical \cite{liu2020learning}. 
A detailed survey can be found in \cite{wang2018deep}.
Although promising results have been achieved in computer vision \cite{hoffman2018cycada} and natural language processing fields \cite{he2016dual}, recent works observe the negative transfer phenomenon when there is little overlap or even conflict knowledge between domains \cite{wang2018deep}. 
For example, such phenomenon will exacerbate in time series fields \cite{hu2020datsing} since time series date indeed show temporal relations while also can be divided into distinct regimes. %That may be one obstacle to consider the time series forecasting from a distribution generalization way.
The mainstream approaches in domain adaptation adopt a parameter-sharing strategy across different domains within a single model.
However, the single model results in stable adaptation at the expense of being incompatible with sudden drift or irregular shift patterns. 
Another drawback is the requirement of accumulating the whole sequential data for training, which may not be realistic due to memory buffer limitations or privacy constraints Besides, defining a domain is not straightforward in non-stationary evolving data since the large cost of domain annotation efforts. There are some interesting and worth-learned works that studied DA without knowing the domain labels by clustering with the style features for image data \cite{kang2019contrastive}. However, that work is designed for image specifically and can not be applied to a more general evolving data setting. In addition, it is not end-to-end trainable due to pre-processing. In contrast, we propose a new end-to-end framework that is capable of avoiding negative transfer by dynamic parameter routes and we can also detect the domain shift simultaneously.
%Based on the assumption of covariate shift \cite{} that the output distribution or labels remain the same when input distribution changes, domain adaptation methods have achieved promising results in computer vision (CV) and natural language processing (NLP) fields \cite{}. Most realistic CV and NLP tasks follow covariate shift assumption due to the semantic consistency property \cite{}, while recent works observe the negative transfer phenomenon when there is little overlap or even conflict knowledge between domains. Such phenomenon will exacerbate in time series fields since time series date indeed show temporal relations while also can be divided into distinct regimes. That may be one obstacle to consider the time series forecasting from a distribution generalization way. Besides, defining a domain
%is not straightforward in non-stationary time series since the data distribution shifts over time \cite{}. There are some interesting and worth-leaning works that studies DA without knowing the domain labels by clustering with the style features for image data \cite{}. However, that work is not applied to time series and it is not end-to-end trainable due to clustering. In contrast, we propose a new end to end framework that is capable of avoiding negative transfer by dynamic parameter routes and we detect the domain shift simultaneously.




%Although there are various models for time-series forecasting, they often suffer from non-stationary time-series, where the data distribution changes over time. Domain adaptation is a common way to alleviate distribution shift and attempts to learn an invariant feature embedding which can reduce the gap between source and target domains. Based on the assumption of covariate shift \cite{} that the output distribution or labels remain the same when input distribution changes, domain adaptation methods have achieved promising results in computer vision (CV) and natural language processing (NLP) fields \cite{}. Most realistic CV and NLP tasks follow covariate shift assumption due the semantic consistency property \cite{}, while recent works observe the negative transfer phenomenon when there is little overlap or even conflict knowledge between domains. Such phenomenon will exacerbate in time series fields since time series date indeed show temporal relations while also can be divided into distinct regimes. That may be one obstacle to consider the time series forecasting from a distribution generalization way. Besides, defining a domain
%is not straightforward in non-stationary time series since the data distribution shifts over time \cite{}. There are some interesting and worth-leaned works that studies DA without knowing the domain labels by clustering with the style features for image data \cite{}. However, that work is not applied to time series and it is not end-to-end trainable due to clustering. In contrast, we propose a new end to end framework that is capable of avoiding negative transfer by dynamic parameter routes and we detect the domain shift simultaneously.
\subsection{Continual Learning}
Continual learning \cite{nguyen2017variational} is another paradigm for sequentially arriving data. 
It avoids revisiting historical data and aims to balance the plasticity-stability dilemma \cite{maracani2021recall}. 
Methods in this domain can be broadly classified into three categories: 
1) replay-based method which stores a small set of historical data or builds a generative model to generate synthetic data for data replay \cite{rolnick2019experience,maracani2021recall};
2) regularization-based method which preserves previous information by penalizing dramatic important parameter changes \cite{ahn2019uncertainty,nguyen2017variational};
3) parameter isolation-based method which balances the plasticity-stability dilemma with a dynamic model architecture \cite{ostapenko2021continual,qin2021bns}. 
This family dedicates different model parameters to each distribution to alleviate forgetting.
Freezing previous model parameters, one can grow new branches for each new data without the consideration of architecture size \cite{nguyen2017variational}. 
Typically, the incremental model architecture enriches the parameter space, hence increasing the capacity to handle the boundlessly shifted distribution. 
However, model size is a big concern in this direction \cite{fini2020online}. 
Our work is more related to the third group in that we learn a dynamic model architecture for adapting to shifted data. 
Different from the mainstream works in the third category, we learn an adaptive sparse network from a whole network. Besides, most CL methods require task information during the training stage. In our work, we consider the adaptation of evolving sequential data where no shift boundary is given.
%When no constraints apply to architecture size, one can grow new branches for new tasks, while freezing previous task parameters [64], [65], or dedicate a model copy to each task [5]. Alternatively, the architecture remains static, with fixed parts allocated to each task

\subsection{Dynamic Linear Models With Switching }
We introduce a discrete variable to detect distribution change for sequentially evolving data, this idea is loosely connected to the topic of switching linear dynamical systems (SLDS) \cite{barber2006expectation,linderman2017bayesian} or change point detection \cite{aminikhanghahi2017survey}. SLDS assumes real-world systems follow a finite number of operating modes or regimes, and each regime is described by linear dynamics and additive Gaussian noise \cite{linderman2017bayesian}. To effectively infer the change point, \cite{dong2020collapsed} proposes a variational inference network and performs exact marginalization of the discrete latent variables. Based on this, \cite{ansari2021deep} introduces a Recurrent Explicit Duration Switching Dynamical System that is capable of identifying both state and time-dependent switching dynamics.
Instead, we allow non-linear regimes described by neural networks and incorporate a discrete variable to solve the distribution shift problem, that can detect multiple distributions rather than a binary one \cite{aminikhanghahi2017survey}.



